Exploring Deep Learning Methods for Real-Time Surgical Instrument Segmentation in Laparoscopy

Minimally invasive surgery is a surgical intervention used to examine the organs inside the abdomen and has been widely used due to its effectiveness over open surgery. Due to the hardware improvements such as high definition cameras, this procedure has significantly improved and new software methods have demonstrated potential for computer-assisted procedures. However, there exists challenges and requirements to improve detection and tracking of the position of the instruments during these surgical procedures. To this end, we evaluate and compare some popular deep learning methods that can be explored for the automated segmentation of surgical instruments in laparoscopy, an important step towards tool tracking. Our experimental results exhibit that the Dual decoder attention network (DDANet) produces a superior result compared to other recent deep learning methods. DDANet yields a Dice coefficient of 0.8739 and mean intersection-over-union of 0.8183 for the Robust Medical Instrument Segmentation (ROBUST-MIS) Challenge 2019 dataset, at a real-time speed of 101.36 frames-per-second that is critical for such procedures.

==> cutout.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure} []
%     \centering
%     \includegraphics[width=5cm, height=6cm]{figures/nasnet_mobile.png}
%     \caption{Proposed architecture.}
%     \label{fig:learning_curve}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure} 
%     \centering
%     \includegraphics[width=5cm, height=5cm]{figures/figure1.png}
%     \caption{Decoder Block} 
%     \label{fig:learning_curve}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure} []
%     \centering
%     \includegraphics[width=5cm, height=6cm]{figures/residual.png}
%     \caption{Residual block}
%     \label{fig:learning_curve}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In the encoder part of the network, RASNet uses the pre-trained ResNet50 model~\cite{he2016deep}, which is trained on ImageNet~\cite{deng2009imagenet}. The decoder part of the network consists of an attention fusion module along with a decoder block. Experimental results on the binary segmentation task of the 2019 Robust Medical Instrument Segmentation (ROBUST-MIS) challenge shows promising results and highlights the potential of reaching the goal of an automated computer-assisted intervention system in the near future. Moreover, our results provide baseline performance on a publicly available dataset. 

%%%%%today%%%%%%%%%


Our previous approach on multi-class endoscopic image classification~\cite{thambawita2020extensive,thambawita2018medico} and endoscopic polyp segmentation~\cite{jha2020kvasir} showed that \ac{CNN} based approach are better than traditional \ac{ML} based approach.
